Universal Shape Replicators via Self-Assembly with Attractive and Repulsive Forces

We show how to design a universal shape replicator in a self-assembly system with both attractive and repulsive forces. More precisely, we show that there is a universal set of constant-size objects that, when added to any unknown hole-free polyomino shape, produces an unbounded number of copies of that shape (plus constant-size garbage objects). The constant-size objects can be easily constructed from a constant number of individual tile types using a constant number of preprocessing self-assembly steps. Our construction uses the well-studied 2-Handed Assembly Model (2HAM) of tile self-assembly, in the simple model where glues interact only with identical glues, allowing glue strengths that are either positive (attractive) or negative (repulsive), and constant temperature (required glue strength for parts to hold together). We also require that the given shape has specified glue types on its surface, and that the feature size (smallest distance between nonincident edges) is bounded below by a constant. Shape replication necessarily requires a self-assembly model where parts can both attach and detach, and this construction is the first to do so using the natural model of negative/repulsive glues (also studied before for other problems such as fuel-efficient computation); previous replication constructions require more powerful global operations such as an "enzyme" that destroys a subset of the tile types.

==> definitions/definitions.tex <==

\section{Definitions and Model}\label{sec:definitions}
\begin{figure*}
	\begin{center}
	\includegraphics[scale=1.0]{definitions/modelex}
	\caption{ This figure introduces our notation for our constructions, as well as a simple example of combination and detachment events.  We denote positive glues with vertical and horizontal lines protruding from tile edges along with numbers and labels denoting glue strength and type.  Negative strength glues are labeled with slanted lines.  Finally, bonded glues between adjacent tiles are depicted with a number denoting the bond strength inscribed within a box between the bonded tile edges.  (a) The 3-tile assembly on the left and the singleton gray tile are combinable into a $2\times 2$ square shown in (b) as the cut between the 2 assemblies yields strength 1.  Note, however, that the producible $2\times 2$ square in (b) is not stable and is breakable into the assemblies shown in (c).
	\label{fig:modelex} }
	\end{center}
\end{figure*}

In this section we first define the two-handed tile self-assembly model with both negative and positive strength glue types and diagonal glue functions.  We also formulate the problem of designing a tile assembly system that replicates an input shape.

\subsection{Tile Self-Assembly Model}
\paragraph{Tiles.}  Consider some alphabet of glue types $\Pi$.  A tile is a finite edge polygon with some finite subset of border points each assigned some glue type from $\Pi$.  Further, each glue type $g \in \Pi$ has some integer number strength $str(g)$.  Finally, each tile may be assigned a finite length string \emph{label}.  In this paper we consider a special class of tiles that are unit squares of the same orientation with at most one glue type per face, with each glue being placed exactly in the center of the tile's face.

\paragraph{Assemblies.}  An assembly is a set of tiles whose interiors do not overlap.  For a given assembly $\Upsilon$, define the \emph{bond graph} $G_\Upsilon$ to be the weighted graph in which each element of $\Upsilon$ is a vertex, and each edge weight between tiles is the sum of the strengths of the overlapping, matching glue points of the two tiles.  An assembly $C$ is said to be \emph{stable} if the bond graph $G_C$ has min-cut at least 1, and \emph{unstable} if the min-cut is less than 1. Note that only overlapping glues that are the same type contribute a non-zero weight, whereas overlapping, non-equal glues always contribute zero weight to the bond graph.  The property that only equal glue types interact with each other is referred to as the \emph{diagonal glue function} property and is perhaps more feasible for experimental implementation than more general glue functions.  Additionally, with the square tiles considered in this paper, stable assemblies will necessarily consist of tiles stacked face to face, forming a subset of the 2D grid.

For an assembly $A$, let $A^*$ denote the set of all assemblies that are equal to $A$ up to translation.  For a set of assemblies $T$, let $T^*$ denote the set of all assembly sets $A^*$ such that $A\in T$.  Put another way, $T^*$ is a set that represents a set of assemblies $T$ if we do not care about translation.


\paragraph{Breakable Assemblies.}
For an (unstable) assembly $C$ whose bond graph $G_C$ has a cut into assemblies $A$ and $B$ with weight less than 1, we say that $C$ is \emph{breakable} into $A$ and $B$.

\paragraph{Combinable Assemblies.}
Informally, two assemblies $A$ and $B$ are said to be combinable into an assembly $C$ if the assemblies can be translated together in such a way that they do not overlap and the sum of the matched glue strengths between the two assemblies is at least 1. Formally, consider two assemblies $A$ and $B$.  If $B$ can be translated into $B'$ such that $C= A \bigcup B'$ is a valid (not overlapping) assembly such that the cut of $G_{A\bigcup B'}$ into $A$ and $B'$ has strength at least 1, then we say that $A$ and $B$ are \emph{combinable} into $C$.

Note that $A$ and $B$ may be combinable into an assembly that is not stable.  This is a key property that is leveraged throughout our constructions.  See Figure~\ref{fig:modelex} for an example.

\paragraph{Producible Assemblies.}
A set of initial assemblies $T$ has an associated set of \emph{producible} assemblies, $\texttt{PROD}_T$, which define what assemblies can grow from the initial set $T$ by any sequence of combination and break events. Formally, $T \subseteq \texttt{PROD}_T$ as a base case set of producible assemblies.  Further, given any $A,B \in \texttt{PROD}_T$ with $A$ and $B$ combinable into $C$, then $C \in \texttt{PROD}_T$, and for any $C \in \texttt{PROD}_T$ where $C$ is breakable into $A$ and $B$, then $A,B \in \texttt{PROD}_T$.  Put another way, the set of producible assemblies contains any assembly that can be obtained by a valid sequence of combinations and breaks, starting from the initial set of assemblies $T$.  We further define the set of \emph{terminal} assemblies, $\texttt{TERM}_T$, to be the subset of $\texttt{PROD}_T$ such that no element of $\texttt{TERM}_T$ can undergo a break or combination transition with another element of $\texttt{PROD}_T$.

Typically, we require that an initial assembly set consist only of stable assemblies.  When $T$ consists only of assemblies that are singleton tiles, $T$ is called a \emph{tile set}.



\subsection{Additional Definitions}

\paragraph{Valid Assembly Sequence.}  For an initial assembly set $T$, a valid assembly sequence for $T$ is any sequence of assemblies $S=\langle a_1, \ldots a_k \rangle$ such that each $a_i \in \texttt{PROD}_T$, and for each $i$ from 1 to $k-1$, $a_i$ is either combinable with some $b \in \texttt{PROD}_T$ to form $a_{i+1}$, or $a_i$ is breakable into $a_{i+1}$ and $b$ for some assembly $b$.  In addition, a valid assembly sequence $S$ is said to be \emph{$\ell$-focused} for label $\ell$ if each assembly in $S$ contains at least one tile with label $\ell$.  A valid assembly sequence is said to be \emph{nascent} if $a_1 \in T$.

For a given partial function $f: \texttt{PROD}_T \rightarrow V$ for a set $V$, define function $f'( \langle a_1,\ldots a_k \rangle )$ to be a function from assembly sequences over $\texttt{PROD}_T$ to sequences over $V$ defined by replacing each $a_i$ with $f(a_i)$ if $f(a_i)$ is defined, and deleting $a_i$ if $f(a_i)$ is not defined.



==> definitions/definitions_new.tex <==
\section{Definitions and Model}\label{sec:definitions}

\begin{figure*}
	\begin{center}
	\includegraphics[width=.70\textwidth]{definitions/modelex2}
	\caption{ This figure introduces notation for our constructions, as well as a simple example of attachment and detachment events. On each tile, the glue label is presented. Red (shaded) labels represent negative glues, and the relevant glue strengths for the tiles can be found in the captions. For caption brevity, for a glue type $X$ we denote $str(X)$ simply as $X$ (e.g. $X + Y = str(X) + str(Y)$). In this temperature $\tau=1$ example, $X = 2$, $Y=1$, $Z=2$ and $N=-1$. (a) The three tile assembly on the left attaches with the single tile with strength $Z + N = 2  - 1 = \tau$ resulting in the $2\times2$ assembly shown in (b). However, this $2\times2$ assembly is unstable along the cut shown by the dotted line, since $Y + N = 1 - 1 < \tau$. Then the assembly is breakable into the assemblies shown in (c).
\label{fig:modelex} }
%This figure introduces our notation for our constructions, as well as a simple example of combination and detachment events.  We denote positive glues with vertical and horizontal lines protruding from tile edges along with numbers and labels denoting glue strength and type.  Negative strength glues are labeled with slanted lines.  Finally, bonded glues between adjacent tiles are depicted with a number denoting the bond strength inscribed within a box between the bonded tile edges.  (a) The 3-tile assembly on the left and the singleton gray tile are combinable into a $2\times 2$ square shown in (b) as the cut between the 2 assemblies yields strength 1.  Note, however, that the producible $2\times 2$ square in (b) is not stable and is breakable into the assemblies shown in (c).

	\end{center}
\end{figure*}

In this section we first define the two-handed tile self-assembly model with both negative and positive strength glue types and diagonal glue functions.  We also formulate the problem of designing a tile assembly system that replicates any input shape.

\subsection{Tile Self-Assembly Model}
\textbf{Tiles.}  Consider some alphabet of glue types $\Pi$.  A tile is a finite edge polygon with some finite subset of border points each assigned some glue type from $\Pi$.  Further, each glue type $g \in \Pi$ has some integer number strength $str(g)$.  Finally, each tile may be assigned a finite length string \emph{label}.  In this paper we consider a special class of tiles that are unit squares of the same orientation with at most one glue type per face, with each glue being placed exactly in the center of the tile's face.

\textbf{Assemblies.}  An assembly is a set of tiles whose interiors do not overlap.  For a given assembly $\Upsilon$, define the \emph{bond graph} $G_\Upsilon$ to be the weighted graph in which each element of $\Upsilon$ is a vertex, and each edge weight between tiles is the sum of the strengths of the overlapping, matching glue points of the two tiles.  For a \emph{temperature} $\tau \in \mathbb{Z}^+$, an assembly $C$ is said to be \emph{stable} if the bond graph $G_C$ has min-cut at least $\tau$, and \emph{unstable} if the min-cut is less than $\tau$. Note that only overlapping glues that are the same type contribute a non-zero weight, whereas overlapping, non-equal glues always contribute zero weight to the bond graph.  The property that only equal glue types interact with each other is referred to as the \emph{diagonal glue function} property and is perhaps more feasible for experimental implementation than more general glue functions. Additionally, with the square tiles considered in this paper, stable assemblies will necessarily consist of tiles stacked face to face, forming a subset of the 2D grid. For an assembly $A$, let $A^*$ denote the set of all assemblies that are equal to $A$ up to translation. For a set of assemblies $T$, let $T^*$ denote the set of all assembly sets $A^*$ such that $A\in T$.  Put another way, $T^*$ is a set that represents a set of assemblies $T$ if we do not care about translation.


\textbf{Breakable Assemblies.}
For an (unstable) assembly $C$ whose bond graph $G_C$ has a cut into assemblies $A$ and $B$ with weight less than $\tau$, we say that $C$ is \emph{breakable} into $A$ and $B$.

\textbf{Combinable Assemblies.}
Informally, two assemblies $A$ and $B$ are said to be combinable into an assembly $C$ if the assemblies can be translated together in such a way that they do not overlap and the sum of the matched glue strengths between the two assemblies is at least $\tau$. Formally, consider two assemblies $A$ and $B$.  If $B$ can be translated into $B'$ such that $C= A \bigcup B'$ is a valid (not overlapping) assembly such that the cut of $G_{A\bigcup B'}$ into $A$ and $B'$ has strength at least $\tau$, then we say that $A$ and $B$ are \emph{combinable} into $C$.

Note that $A$ and $B$ may be combinable into an assembly that is not stable.  This is a key property that is leveraged throughout our constructions.  See Figure~\ref{fig:modelex} for an example.


\textbf{Assembly States and Tile Systems.}
An \emph{assembly state} is a multiset (finite or infinite) of assemblies. For an assembly state $S$ and an assembly $A$, we use $C(S, A)$ to denote the multiplicity of $A$ in $S$ and $\texttt{supp} S$ to denote the support of $S$ (the set of unique elements in $S$).
%An \emph{assembly state} is an ordered tuple $S = \{\mathcal{A}, \mathcal{M} \}$ where $\mathcal{A}$ is a set of assemblies and $\mathcal{M}$ is a function mapping $\mathcal{A} \rightarrow {\mathbb{N}, \infty}$.
%Further, for any assembly $b \notin \mathcal{A}$, $\mathcal{M}(b)=0$.
%$M(a)$ is referred to as the \emph{multiplicity} of $a$.
A \emph{tile system} is an ordered tuple $\Gamma = \{ \sigma, \tau \}$  where $\sigma$ is an assembly state called the \emph{initial assembly state} and $\tau$ is a positive integer called the \emph{temperature}.
For this work, we constrain assemblies $a\in\sigma$ to be singleton tiles. Then, the tile complexity of $\Gamma$ is $| \texttt{supp} \sigma|$, the number of unique tiles in the initial assembly state.
A tile system has an associated set of \emph{producible} assemblies, $\texttt{PROD}_\Gamma$, which define what assemblies can grow from the initial assemblies in $\sigma$ by any sequence of combination and break events, regardless of multiplicities of the assemblies. Formally, $\texttt{PROD}_\Gamma$ contains all unique elements of $\sigma$ as a base case set of producible assemblies.  Further, given any $A,B \in \texttt{PROD}_\Gamma$ with $A$ and $B$ combinable into $C$, then $C \in \texttt{PROD}_\Gamma$, and for any $C \in \texttt{PROD}_\Gamma$ where $C$ is breakable into $A$ and $B$, then $A,B \in \texttt{PROD}_\Gamma$.  Put another way, the set of producible assemblies contains any assembly that can be obtained by a valid sequence of combinations and breaks, starting from the initial set of assemblies in $\sigma$.  We further define the set of \emph{terminal} assemblies, $\texttt{TERM}_\Gamma$, to be the subset of $\texttt{PROD}_\Gamma$ such that no element of $\texttt{TERM}_\Gamma$ can undergo a break or combination transition with another element of $\texttt{PROD}_\Gamma$.




%Typically, we require that an initial assembly set consist only of stable assemblies.  When $T$ consists only of assemblies that are singleton tiles, $T$ is called a \emph{tile set}.



%\subsection{Additional Definitions}

\textbf{Valid Assembly State Sequences.}
Informally, a valid assembly state sequence of a tile system is a sequence of assembly states in which each subsequent state consists of 1 break or combination of assemblies from the previous state, including the appropriate increase or decrease in multiplicity of the assemblies.
Formally, for a tile system  $\Gamma = \{ \sigma, \tau \}$, a valid assembly state sequence is any sequence of assembly states $\mathcal{S}=\langle S_1, S_2, \ldots S_k \rangle$ such that for each $i$ from 1 to $k-1$, either $S_{i+1} \setminus S_i$ contains exactly one assembly $C$ such that there exist $A, B\in S_i \setminus S_{i+1}$ that are combinable into $C$ or $S_{i+1} \setminus S_i$ contains exactly two assemblies $A$ and $B$ such that there exists $C\in S_i \setminus S_{i+1}$ such that $C$ is breakable into $A$ and $B$. In other words, in each subsequent assembly state in the sequence, the difference in states is exactly one attachment or detachment event. Additionally, $S_1 = \sigma$, meaning the assembly state sequence begins at the initial assembly state.
%such that for each $S_i = \{\mathcal{A}_i, \mathcal{M}_i\}$ from $S_1$ to $S_{k-1}$, exactly one of the following is true:
%\begin{itemize}
%\item There exist assemblies $A, B \in \mathcal{A}_i$ such that $A$ and $B$ are combinable into $C\in\mathcal{A}_{i+1}$ with $\mathcal{M}_i(C)+1 = \mathcal{M}_{i+1}(C)$, $\mathcal{M}_{i}(A)-1 = \mathcal{M}_{i+1}(A),
%\end{itemize}
%each $S_i \in \texttt{PROD}_T$, and for each $i$ from 1 to $k-1$, $a_i$ is either combinable with some $b \in \texttt{PROD}_T$ to form $a_{i+1}$, or $a_i$ is breakable into $a_{i+1}$ and $b$ for some assembly $b$.  In addition, a valid assembly sequence $S$ is said to be \emph{$\ell$-focused} for label $\ell$ if each assembly in $S$ contains at least one tile with label $\ell$.  A valid assembly sequence is said to be \emph{nascent} if $a_1 \in T$.

%For a given partial function $f: \texttt{PROD}_T \rightarrow V$ for a set $V$, define function $f'( \langle a_1,\ldots a_k \rangle )$ to be a function from assembly sequences over $\texttt{PROD}_T$ to sequences over $V$ defined by replacing each $a_i$ with $f(a_i)$ if $f(a_i)$ is defined, and deleting $a_i$ if $f(a_i)$ is not defined.

\subsection{Shape Replication Systems}

\textbf{Shapes and Valid Input Assemblies}
 For a given stable assembly $\Upsilon$, let $S_\Upsilon$, denote the set of positions ($i$, $j$) for each of the tiles of $\Upsilon$. A \emph{shape} is a connected subset of the 2D grid. For a given shape $S$, let $S^*$ denote the set of all shapes equal to $S$ up to translation. $\Upsilon$ is said to have shape $S$ \emph{iff} $S_\Upsilon \in S^*$.
A \emph{valid input assembly} for a tile system $\Gamma = \{\sigma, \tau\}$ is a stable assembly \emph{iff} all north, east, west, and south facing edges along its perimeter have glues of $N, E, S,$ and $W$, respectively, with the exception of the westmost northmost positioned tile having a north glue of $C1$ glue and west glue of $C2$.

\textbf{Unbounded Replication System.}
An \emph{unbounded replication system} is a tile system $\Gamma = \{\sigma, \tau\}$ such that, given a valid input assembly $X$ (with its shape to be replicated), for any $n\in \mathbb{N}$, for each valid assembly sequence of $\Gamma' = \{\sigma\cup{X}, \tau\}$ either there exists an assembly state $M_{done}$ such that, for an assembly $X'$ with shape $S_X$, $C(M_{done}, X') = n$ or the valid assembly sequence of $\Gamma'$ is a subsequence of some valid assembly state sequence $Q$ in which there exists such an assembly state. That is, for any number, the replication system generates at least that many \emph{copies} of $X$. The \emph{terminal garbage size} of the system is $\max_{|A|} A\in \texttt{TERM}_\Gamma$ such that $A$ does not have shape $S_X$. The \emph{size of producibles} for the system is $\max_{|A|} A\in \texttt{PROD}_\Gamma$.
% An \emph{unbounded replication system} is a tile system $\Gamma = \{\sigma, \tau\}$ such that, given a valid input assembly $X$ with shape $S_X$ (to be replicated), for any $n\in \mathbb{N}$, for each valid assembly sequence of $\Gamma' = \{\sigma\cup{X}, \tau\}$ either there exists an assembly state $S_{done}$ such that, for an assembly $X'$ with shape $S_X$, $C(S_{done}, X') = n$ or the valid assembly sequence of $\Gamma'$ is a subsequence of some valid assembly state sequence $S$ in which there exists such an assembly state. That is, for any number, the replication system generates at least that many copies of $X$. The \emph{terminal garbage size} of the system is $\max_{|A|} A\in \texttt{TERM}_\Gamma$ such that $A$ does not have shape $S_X$. The \emph{size of producibles} for the system is $\max_{|A|} A\in \texttt{PROD}_\Gamma$.


%\paragraph{Precise Count Replication System.}
%A \emph{precise $n$-count replication system} is a tile system $\Gamma = \{\sigma, \tau\}$ such that, given a valid input assembly $X$ with shape $S_X$ (to be replicated), each valid assembly sequence of $\Gamma' = \{\sigma\cup{X}, \tau\}$ is a subsequence of some valid assembly sequence in which there exists an assembly state $S_{done}$ such that, for an assembly $X'$ with shape $S_X$, $C(S_{done}, X') = n$. That is, given any number, the replication system generates exactly that many copies of $X$. The \emph{terminal garbage size} of the system is $\max_{|A|} A\in \texttt{TERM}_\Gamma$ such that $A$ does not have shape $S_X$. The \emph{size of producibles} for the system is $\max_{|A|} A\in \texttt{PROD}_\Gamma$.


==> introduction/stuffToCite.tex <==
\subsection{Stuff to Cite}
Information replication in crystal growth in tile self-assembly
\cite{SCHUL2012}

Shape replication in staged RNA model:
\cite{Abel:2010:SRT:1873601.1873686}

Pattern Replication in signal tile model:
\cite{keenan14exponential}
(also nice references to von Neumann etc.)

Shape replication in signal tile model:
\cite{Hendricks2015}

2HAM in 3D simulating 2D signal passing without glue deactivation or assembly breaking:
\cite{Fochtman2015}

Negative glues aTAM (rgTAS = one $-1$ glue, rest $+1$), temperature 1 computation
\cite{rgTAM}

Negative glues aTAM (non-diagonal glue matrix!), space efficient computation
\cite{DotKarMas10}

Negatives glues 2HAM, fuel-efficient computation:
\cite{SS2013FEC}

Negative glues 2HAM (rg2HAM with glues $\{-1,0,1\}$), temperature 1, computation
\cite{PRS2016RMN}



==> introduction/table.tex <==
\begin{center}
\begin{tabular}{| c | c | c | c |}
  \hline			
  Replication Count & Tile Complexity & Terminal Garbage Size & Size of Producibles \\ \hline
  Unbounded & $\mathcal{O}(1)$ & $\mathcal{O}(1)$ & $\mathcal{O}(|S|)$ \\ \hline
  $n$ & $\mathcal{O}(\log n)$ & $\mathcal{O}(n\log n)$ & $\mathcal{O}(\max{(|S|, n \log n)})$ \\
  \hline
\end{tabular}
\end{center} 

==> preciseCount.tex <==
\begin{theorem}
Given $n\in\mathbb{N}$, there exists a precise $n$-count shape replication system $\Gamma = \{  \sigma, 100 \}$ with $\mathcal{O}(\log n)$ tile complexity, $\mathcal{O}(n\log n)$ terminal garbage size, and $\mathcal{O}(\max{(|S|,n \log n)})$ size of producibles where $S$ is the input assembly.
\end{theorem} 
